Azimuth: Systematic Error Analysis for Text Classification

We present Azimuth, an open-source and easy-to-use tool to perform error analysis for text classification. Compared to other stages of the ML development cycle, such as model training and hyper-parameter tuning, the process and tooling for the error analysis stage are less mature. However, this stage is critical for the development of reliable and trustworthy AI systems. To make error analysis more systematic, we propose an approach comprising dataset analysis and model quality assessment, which Azimuth facilitates. We aim to help AI practitioners discover and address areas where the model does not generalize by leveraging and integrating a range of ML techniques, such as saliency maps, similarity, uncertainty, and behavioral analyses, all in one tool. Our code and documentation are available at github.com/servicenow/azimuth.

==> ReviewerComments.tex <==
REVIEWER #1 
No proposed improvements

REVIEWER #2
The paper could be further strengthened by: 

1. providing some justification for the choice of component methods (e.g. why saliency maps in particular for explainability)
- Very good point. We added some justification under Syntax Analysis and Explainability.

2.  some discussion of the extent to which the architecture might permit the introduction of additional approaches.
- Thank you for the suggestion. We added a small section 3.5 Extensibility, where we point to further documentation under our Github repo.

3. The behavioral analysis component also seems a bit underdeveloped relative to the test case driven vision proposed by Ribeiro and colleagues, and one wonders if the authors might consider expanding this component to accommodate customized capability-specific perturbations.
- Indeed, we only scratch the surface of what can be done with the CheckList paradigm. We added language to indicate that what we provide in Azimuth is basic and users can add new functions to cover more of what Ribeiro et. al propose.

4. Finally, while it is encouraging to see that collaborative design was used to iteratively improve the system, it would be helpful to know if any problems were identified in the initial stages of this design process (the current description refers only to the resulting improvements).
- This is a great idea. Due to space limitations, we were only able to add a few lines in the Design section in the main body of the paper, but we have added a substantial amount of detail in a new section in Appendix A (A.3 Design Challenges).


REVIEWER #3

The issues I see are the following:

1) lack of concrete detail and examples in the body of the paper.

The main complaint I have about this paper is that we only see specific examples of the types of analyses available within Azimuth when we get to the appendix. The paper would be far more compelling if the examples were in the body of the text rather than the appendix. Even within the appendix, some of the illustrations (specifically Figure 7 and Figure 8) show features of the software (e.g. the ability to select columns to hide) without showing or explaining how these features might influence the analysis. Figure 7 shows the filtering dashboard, but it's not really clear from the image what's happening here, and there's no concrete explanation.
- Thank you for pointing this out! We have added section 3.1 User Workflow to address this as well as expanded the 3.3 Capabilities section, particularly by adding more examples of use cases and areas of implementation.

As another example, the design section is quite vague and lacking concrete detail - it would be better to use that space to show examples of the various analyses.
- We agree that more detail and examples would be compelling and support the rest of the text, but have struggled with how to convey the importance of design in the development of Azimuth given space limitations. Our compromise was to make the main points in section 3.4 Design while elaborating in Appendix A. However, as mentioned above, in this revision, we have also added information on design challenges encountered in user interviews and their solutions, both in the main Design section and in the Appendix.

2) The authors criticize "current common error analysis practices" without properly explaining what those are - it's hard to know precisely what capabilities they're comparing to and improving upon.
- We have softened the language to say "the current common error analysis practices may not be sufficiently thorough to provide this visibility, limiting our capacity to build safe, trustworthy AI systems". We note that more details on current common error analysis practices are also presented later on in the introduction.

At the same time, we feel there has not been enough research into the error analysis stage of ML product development and therefore our assessment comes from our experience in industry and the experience of colleagues in the NLP community. 

3) The paper makes some strange claims about "academic datasets" (whatever that even means). Consider either softening the claims or explaining them in greater detail.
- Thank you for raising this. Most of us have experience in both academia and industry, where we are trying to ship AI-based products. We see significant differences between datasets that are generally used in academic publications and the real, unpredictable data that user-generated traffic generates. We have softened the claim to avoid misunderstandings.

Some other, more minor issues and suggestions appear below, in the "Questions" field.

Overall, I would consider accepting this paper if the revisions described above can be made, and if the emphasis of the writing shifts in the direction of detailed, concrete illustrations of the analyses available and the insights they can provide.

Questions for Authors
Comments:
1. Figure 1 is too small and not adequately explained - it doesn't give me a good sense of the system's main capabilities - would be helpful to briefly explain the task, at a minimum
- We added a new section 'User Workflow' where we detail the different screens, including the one captured in Figure 1. We also added other screenshots of the system's capabilities along with a description.

2. The heading "annotation artifacts" under model quality assessment is slightly misleading - this is more about model overreliance on annotation artifacts, not about the artifacts themselves
Figure 2 is quite nice!
- Wherever possible, we have changed the heading to "Annotation Artifacts Discovery" to emphasize that we want to help users discover them.

Qs:

1. imbalance is a natural attribute of many NLP datasets -- can tool account for this somehow?
- The current version simply allows users to specify at what point class imbalance is problematic. Since this is task- and user-dependent, we do not have an obvious solution that would cover most scenarios.
2. can the system perform the suggested resolutions? (for dataset quality issues) - that would be very useful!
- We agree that this would be very useful. We are considering this as future work!
3. how is class imbalance determination implemented? (in other words, is there a specific threshold? is it configurable?)
- All thresholds are configurable. Details on how the warnings are computed can be found in our documentation here: https://servicenow.github.io/azimuth/main/user-guide/dataset-warnings/.

4. is syntax analysis more than sentence length? b/c that's not syntax
- It is more than sentence length; we leverage dependency trees and part-of-speech tags to create smart tags. We have added content under section 3.3 Capabilities to explain this further.

5. what are the "small perturbations" performed for data augmentation/behavioral analysis? 
- We detail all tests in our documentation here: https://servicenow.github.io/azimuth/main/key-concepts/behavioral-testing/. We also added details in the paper about the types of tests that we implemented, which are Robustness Invariance tests.
